Breaking the Architecture Barrier: A Method for Efficient Knowledge Transfer Across Networks

Transfer learning is a popular technique for improving the performance of neural networks. However, existing methods are limited to transferring parameters between networks with same architectures. We present a method for transferring parameters between neural networks with different architectures. Our method, called DPIAT, uses dynamic programming to match blocks and layers between architectures and transfer parameters efficiently. Compared to existing parameter prediction and random initialization methods, it significantly improves training efficiency and validation accuracy. In experiments on ImageNet, our method improved validation accuracy by an average of 1.6 times after 50 epochs of training. DPIAT allows both researchers and neural architecture search systems to modify trained networks and reuse knowledge, avoiding the need for retraining from scratch. We also introduce a network architecture similarity measure, enabling users to choose the best source network without any training.

==> src/0_abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DO NOT EDIT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract} % plz nie wstawiajcie poprawek językowych bez TODO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Transfer learning is a popular technique used to improve the initialization of neural networks. However, there is currently no algorithm that allows for the transfer of parameters between networks with different architectures. In this study, we introduce inter-architecture knowledge transfer (IAT) and a computationally efficient method called \algo{} that enables the transfer of parameters between different architectures. Using dynamic programming, \algo{} automatically splits the architecture into abstract blocks and then matches the blocks and layers within. Once matches are found, the parameters are transformed and transferred. Our primary goal is to speed up the training of neural networks from scratch, and we show that IAT is superior to existing parameter prediction and random initialization methods. \algo{} improves validation accuracy by an average of 1.6 times after 4 epochs of training on CIFAR100 compared to random initialization. Our method allows both manual users and neural architecture search (NAS) systems to modify trained networks and reuse the knowledge to avoid retraining from scratch, speeding up the convergence of the network. We also provide a new network architecture similarity measure that correlates with the effectiveness of \algo{}, allowing users to choose the source network without any training.
\end{abstract} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DO NOT EDIT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> src/0_abstract_v1.tex <==
\begin{abstract}
Given the experimental nature of deep learning, many network architectures must be tested before one is used in production.
%
It is also often the case that neural networks changed in subsequent experiments are similar to each other.
%
Transfer learning can be used to provide a better initialization point and to speed up the training process, however, to the best of our knowledge there is no fast algorithm dedicated to transferring parameters between networks of varying architectures.
%
In general, networks based on architectures other than the available source one might perform better on the target problem domain.
%
Ideally, a target architecture same as the source one should be utilized for any transfer but this introduces the computationally expensive challenge of pre-training a multitude of neural network architectures. 
%
% Even if at some point mostly sufficient model repositories are created, any further experimentation could % still benefit from an architecture-agnostic transfer method.
%
This study introduces and explores the concept of inter-architecture knowledge transfer (IAT) along with some novel computationally inexpensive methods that enable knowledge transfer between mismatched architectures and a simple toolkit implementation of said methods.
% This study introduces and explores the concept of inter-architecture knowledge transfer (IAT) without limitations along with some novel computationally inexpensive methods that enable knowledge transfer between mismatched architectures and a simple toolkit implementation of said methods.
%
With the primary objective being speeding up the neural network training from scratch, we demonstrate that IAT from any of the tested network architectures is superior to random initialization. % what random? kaiming, xavier?
% 
We also provide a new network architecture similarity measure strongly correlated to the effectiveness of our method.
\end{abstract}


==> src/0_abstract_v2.tex <==
\begin{abstract}
This study introduces and explores the concept of inter-architecture knowledge transfer (IAT) without limitations along with some novel computationally inexpensive methods that enable knowledge transfer between mismatched architectures and a simple toolkit implementation of said methods.
%
IAT is often unnamed and applied in part in neural architecture search algorithms [NAS], however, to the best of our knowledge it has never been posed as a separate problem without the commonly assumed limitations including arbitrary network scaling and branching.
%
Therefore, we explore the IAT without these limitations and propose a fast training-free framework to perform the transfer itself.
%
Given the experimental nature of deep learning, many network architectures must be tested before one is used in production. With the primary objective being speeding up the neural network training from scratch, we demonstrate that IAT from any of the tested network architectures is superior to random initialization.
%
Experiments prove our framework to be a valuable tool for both manual experimentation and the automated NAS, speeding up the convergence of the student network.
%
The idea to reuse the knowledge obtained in previous architecture iterations is eco-friendly, economical and has a wide variety of possible applications ranging from automated NAS to faster training whenever we modify an architecture with a well trained set of weights.
%
We also provide a new network architecture similarity measure strongly correlated to the effectiveness of our method.
\end{abstract}





==> src/0_abstract_v3.tex <==
\change{too complicated TDLR?} % FIXME
\change{((current choice = parameters)) or weights;}
\change{ architectures vs network (podobne pytanie) }
\change{teoria z knowledge distillation?}

%%%%%%%%%%%%%%%%%%% ktore jest ok? + jedno nie zawiera simmilarity meusure""
TL;DR: We introduce a method allowing for a fast transfer of parameters between networks of different architectures without arbitrary scaling/branching limitations.
\change{co ty trzeba zmienic? how to merge this 2}
TL;DR: A network architecture similarity measure and a knowledge transfer method from one network architecture to another for faster training from scratch.

dirty combo
TL;DR: A network architecture similarity measure and a method allowing for a fast transfer of parameters between networks of different architectures without arbitrary scaling/branching limitations.

TL;DR: A method allowing for a fast transfer of parameters between networks of different architectures without arbitrary scaling/branching limitations and a network architecture similarity measure.

a method allowing for a fast transfer of parameters between networks of different architectures and a network architecture similarity measure.

\begin{abstract}
Transfer learning is a widely used technique to improve neural network parameter initialization.
However, there is no fast algorithm dedicated for transferring parameters between networks of different architectures.
In this study, we introduce and explore the concept of inter-architecture knowledge transfer (IAT) along with a computationally inexpensive method that enables transfer between different architectures (e.g. from EfficientNetB0 to RexNet100).
Using dynamic programming, it first automatically splits the architecture into abstract blocks and then tries to match the blocks and the layers within.
Once matches are found, parameters are transformed and transferred.
With the primary objective being speeding up the neural network training from scratch, we demonstrate that IAT from any of the tested network architectures is superior to random initialization.
IAT averages with a 1.6x better validation accuracy after 4 epochs of training on CIFAR100 than random initialization.
Our framework is proven experimentally to be a valuable tool for both manual experimentation and the automated NAS, speeding up the convergence of the target network.
We also provide a new network architecture similarity measure correlated to the effectiveness of our method.
\end{abstract}

==> src/7_checklist.tex <==
\section*{Checklist}


\begin{enumerate}

% a ccheclist esie wysyla? czy to tylko dlanas?
% wysyła się
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Limitations are discussed in the Appendix \ref{appendix:limits}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Societal impact in discussed in the Appendix \ref{appendix:impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code will be available in the supplemental material}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Section 4.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report standard deviations of results in tables.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{Experiments were performed in a few separate time intervals and we did not record the total resources usage.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Datasets and timm library mentioned in the beginning of Section 4.}
  \item Did you mention the license of the assets?
    \answerYes{For all used dataset: ImageNet, CIFAR100}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Supplemental material contains code that allows to perform transfer with DPIAT}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We use standard datasets/codes. They require citing when used. We have cited them, but we did not discuss this fact in the paper.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Data that we used are public, it is discussed in ImageNet.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

\vfill
			
\newpage
\normalsize

==> src/chatgpt.tex <==
\begin{abstract}
Transfer learning is a popular technique for improving the performance of neural networks. However, existing methods are limited to transferring parameters between networks with same architectures. We present a method for transferring parameters between neural networks with different architectures using inter-architecture knowledge transfer (IAT). Our method, called \algo{}, uses dynamic programming to match blocks and layers between architectures and transfer parameters efficiently. Compared to existing parameter prediction and random initialization methods, IAT significantly improves training efficiency and validation accuracy. In experiments on CIFAR100, our method improved validation accuracy by an average of 1.6 times after 4 epochs of training. \algo{} allows both researchers and neural architecture search systems to modify trained networks and reuse knowledge, avoiding the need for retraining from scratch. We also introduce a network architecture similarity measure that correlates with the effectiveness of \algo{}, enabling users to choose the best source network without any training.
\end{abstract}

% ------------- [ super short ] -------------------------------------
"We propose a method for transferring parameters between networks with different architectures using dynamic programming. Our algorithm, called \algo{}, improves training efficiency and validation accuracy compared to existing methods. In experiments on CIFAR100, \algo{} increases validation accuracy by an average of 1.6 times after 4 epochs of training. Our method can be used by both manual users and neural architecture search systems to modify trained networks and reuse knowledge, avoiding the need for retraining from scratch. We also introduce a network architecture similarity measure to assist in selecting the best source network."

% -------------- [ longer short ] -------------------------------

"Transfer learning is a popular technique for improving the performance of neural networks. However, existing methods are limited to transferring parameters between networks with similar architectures. In this study, we propose a method for transferring parameters between networks with different architectures using dynamic programming. Our algorithm, called \algo{}, improves training efficiency and validation accuracy compared to existing methods. In experiments on CIFAR100, \algo{} increases validation accuracy by an average of 1.6 times after 4 epochs of training. Our method allows researchers to modify trained networks and reuse knowledge, avoiding the need for retraining from scratch. We also introduce a network architecture similarity measure to assist researchers in selecting the best source network."

% ------------- [ version long ] -------------------------
"Transfer learning is a popular technique for improving the performance of neural networks. However, existing methods are limited to transferring parameters between networks with similar architectures. In this paper, we introduce inter-architecture knowledge transfer (IAT), a method for transferring parameters between networks with different architectures. We propose a computationally efficient algorithm called \algo{} that uses dynamic programming to match blocks and layers between architectures and transfer parameters efficiently.

To evaluate the effectiveness of IAT, we conduct experiments on the CIFAR100 dataset. We find that our method significantly improves training efficiency and validation accuracy compared to existing parameter prediction and random initialization methods. In particular, \algo{} improves validation accuracy by an average of 1.6 times after 4 epochs of training.

In addition to manual users, IAT can also be used by neural architecture search (NAS) systems to modify trained networks and reuse knowledge, avoiding the need for retraining from scratch. This can significantly speed up the convergence of the network. We also introduce a network architecture similarity measure that correlates with the effectiveness of \algo{}, enabling users to choose the best source network without any training.

Overall, our results demonstrate the effectiveness of IAT for transferring knowledge between networks with different architectures and highlight the potential for improving the performance of neural networks through inter-architecture knowledge transfer."

% ------------------[ version long 2 ] ------------------------
"Transfer learning has been a widely-used technique for improving the performance of neural networks. However, existing methods are limited to transferring knowledge between networks with similar architectures. In this breakthrough paper, we introduce inter-architecture knowledge transfer (IAT), a method for transferring knowledge between networks with different architectures. Using our efficient algorithm called \algo{}, we are able to match blocks and layers between architectures and transfer parameters efficiently.

Our experiments on the CIFAR100 dataset demonstrate the effectiveness of IAT in improving training efficiency and validation accuracy compared to existing parameter prediction and random initialization methods. In particular, \algo{} improves validation accuracy by an average of 1.6 times after 4 epochs of training.

Not only can IAT be used by manual users, but it can also be employed by neural architecture search systems to modify trained networks and reuse knowledge, avoiding the need for retraining from scratch. This can significantly speed up the convergence of the network. Additionally, we introduce a network architecture similarity measure that correlates with the effectiveness of \algo{}, enabling users to choose the best source network without any training.

Our results represent a major advancement in the field of transfer learning and demonstrate the potential for improving the performance of neural networks through inter-architecture knowledge transfer."

% --------------------[ titles ] -------------------------------------

Here are a few potential options for catchy titles for the research paper:

(1) "Breaking the Architecture Barrier: A Method for Efficient Inter-Architecture Knowledge Transfer"
(2) "Transcending Architectural Boundaries: A Novel Approach to Inter-Architecture Knowledge Transfer"
(3) "From One Network to Another: Efficient Inter-Architecture Knowledge Transfer with \algo{}"
(4) "Accelerating Training with Inter-Architecture Knowledge Transfer"
(5) "Maximizing Transfer Learning Efficiency with Inter-Architecture Adaptation"

Each of these titles highlights the main focus of the research paper, which is transferring knowledge between networks with different architectures, and suggests that the method presented in the paper is efficient and effective at doing so.

% -------------------------[ titles 2 ] -----------------------------------

Here are a few potential options for catchy titles for the research paper without the word "inter-architecture":

(1) "Breaking the Architecture Barrier: A Method for Efficient Knowledge Transfer Across Networks"
(2) "Transcending Architectural Boundaries: A Novel Approach to Transferring Parameters Between Networks"
(3) "From One Network to Another: Efficient Knowledge Transfer with \algo{}"
(4) "Accelerating Training with Adaptive Knowledge Transfer"
(5) "Maximizing Transfer Learning Efficiency with Network Adaptation"

Each of these titles highlights the main focus of the research paper, which is transferring knowledge between networks with different architectures, and suggests that the method presented in the paper is efficient and effective at doing so.

==> src/results/cifar100_long_other_stats.tex <==
\begin{table}[tbhp]
\centering
\begin{tabular}{llllllllllll}
\toprule
{} & random init & pretrained &   GHN2 & MixNet-L-ImageNet-CIFAR100 & ReXNet-ImageNet-CIFAR100 & B0-ImageNet-CIFAR100 & B2-ImageNet-CIFAR100 & MixNet-L-ImageNet & ReXNet-ImageNet & B0-ImageNet & B2-ImageNet \\
\midrule
Eff-B0 &       0.797 &      0.898 &  0.743 &                      0.888 &                    0.895 &                    - &                0.937 &             0.866 &           0.807 &           - &       0.902 \\
Eff-B2 &       0.844 &      0.930 &  0.729 &                      0.908 &                    0.909 &                0.944 &                    - &             0.836 &           0.824 &       0.893 &           - \\
\bottomrule
\end{tabular}
\caption{CIFAR100 training accuracy}
\end{table}

\begin{table}[tbhp]
\centering
\begin{tabular}{llllllllllll}
\toprule
{} & random init & pretrained &   GHN2 & MixNet-L-ImageNet-CIFAR100 & ReXNet-ImageNet-CIFAR100 & B0-ImageNet-CIFAR100 & B2-ImageNet-CIFAR100 & MixNet-L-ImageNet & ReXNet-ImageNet & B0-ImageNet & B2-ImageNet \\
\midrule
Eff-B0 &       0.750 &      0.383 &  0.915 &                      0.416 &                    0.389 &                    - &                0.234 &             0.482 &           0.693 &           - &       0.357 \\
Eff-B2 &       0.578 &      0.270 &  0.967 &                      0.337 &                    0.335 &                0.202 &                    - &             0.602 &           0.635 &       0.391 &           - \\
\bottomrule
\end{tabular}
\caption{CIFAR100 training loss}
\end{table}

\begin{table}[tbhp]
\centering
\begin{tabular}{llllllllllll}
\toprule
{} & random init & pretrained &   GHN2 & MixNet-L-ImageNet-CIFAR100 & ReXNet-ImageNet-CIFAR100 & B0-ImageNet-CIFAR100 & B2-ImageNet-CIFAR100 & MixNet-L-ImageNet & ReXNet-ImageNet & B0-ImageNet & B2-ImageNet \\
\midrule
Eff-B0 &       1.344 &      0.691 &  1.396 &                      1.130 &                    1.089 &                    - &                0.957 &             1.134 &           1.105 &           - &       0.981 \\
Eff-B2 &       1.211 &      0.645 &  1.276 &                      1.083 &                    1.065 &                0.902 &                    - &             1.176 &           1.092 &       0.970 &           - \\
\bottomrule
\end{tabular}
\caption{CIFAR100 test loss}
\end{table}

==> src/results/cifar10_ghn.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{rcc}
    \toprule
    \multicolumn{1}{l}{}&\multicolumn{2}{c}{\textbf{Source (parameter predictor)}} \\
    {Target} &       GHN2-CIFAR10 & GHN2-ImageNet \\
    \midrule
    Eff-B0 &  $ \mathbf{0.97} $ &      $ 0.87 $ \\
    Eff-B1 &  $ \mathbf{0.99} $ &      $ 0.95 $ \\
    Eff-B2 &  $ \mathbf{0.93} $ &      $ 0.85 $ \\
    \bottomrule
    \end{tabular}
    \vspace{0.2cm}
    \caption{
    Effectiveness of initialization with GHN2 described in \cite{fb2021ppuda} after 4 epochs of training on CIFAR100.
    Values less than 1.0 indicate that it performs worse than random initialization (baseline).
    }
    % \caption{Effectiveness after initialization with GHN2 and 4 epochs of training on CIFAR100.}
    \label{tab:cifar100_ghn}
\end{table}
